Anisotropic star with a linear equation of state (EOS)

A family of solutions defining the interior of a static, spherically symmetric, compact anisotropic star is described by considering a new form of the equation of state (EOS). The analytic solution is derived by using the Finch and Skea ansatz for the metric potential g_rr, which has a clear geometric interpretation for the related background spacetime. The model parameters are fixed by smooth matching of the interior solution to the Schwarzschild exterior metric over the bounding surface of the compact star, together with the requirement that the radial pressure vanishes at the boundary. Data available for the pulsar 4U1802030 has been utilized to analyze the physical viability of the developed model. The model is shown to be stable.

==> ref.tex <==

\bibitem{nilsson2000general}
Ulf S Nilsson and Claes Uggla;
%\newblock General relativistic stars: Linear equations of state.
\newblock {\em Annals of Physics}, \textbf{286}:278--291, 2000.

\bibitem{ivanov2001relativistic}
B V Ivanov;
%\newblock Relativistic static fluid spheres with a linear equation of state.
\newblock {\em arXiv preprint gr-qc/0107032}, 2001.

\bibitem{maharaj2006equation}
S D Maharaj and M Chaisi;
%\newblock Equation of state for anisotropic spheres.
\newblock {\em General Relativity and Gravitation}, \textbf{192}:1723--1726, 2006.

\bibitem{sharma2007class}
R Sharma and S D Maharaj;
%\newblock A class of relativistic stars with a linear equation of state.
\newblock {\em Monthly Notices of the Royal Astronomical Society},
\textbf{375}:1265--1268, 2007.

\bibitem{thirukkanesh2008charged}
S Thirukkanesh and S D Maharaj;
%\newblock Charged anisotropic matter with a linear equation of state.
\newblock {\em Classical and Quantum Gravity}, \textbf{25}(23):1--14, 2008.

\bibitem{maharaj2009generalized}
S D Maharaj and S Thirukkanesh;
%\newblock Generalized isothermal models with strange equation of state.
\newblock {\em Pramana}, \textbf{72}:481--494, 2009.

\bibitem{varela2010charged}
V Varela, F Rahaman, S Ray, K Chakraborty, and  M Kalam;
%\newblock Charged anisotropic matter with linear or nonlinear equation of
%state.
\newblock {\em Physical Review D}, \textbf{82}:1--14, 2010.

\bibitem{maharaj2014some}
S D Maharaj, J M Sunzu, and S Ray;
%\newblock Some simple models for quark stars.
\newblock {\em The European Physical Journal Plus}, \textbf{129}:1--10, 2014.

\bibitem{ngubelanga2015compact}
S A Ngubelanga, S D Maharaj, and S Ray;
%\newblock Compact stars with quadratic equation of state.
\newblock {\em Astrophysics and Space Science}, \textbf{357}:1--9, 2015.

\bibitem{harko2016exact}
T Harko and M K Mak ;
%\newblock Exact power series solutions of the structure equations of the
%	general relativistic isotropic fluid stars with linear barotropic and
%polytropic equations of state.
\newblock {\em Astrophysics and Space Science}, \textbf{361}:283--302, 2016.

\bibitem{thomas2017anisotropic}
V O Thomas and D M Pandya;
%\newblock Anisotropic compacts stars on paraboloidal spacetime with linear
%equation of state.
\newblock {\em The European Physical Journal A}, \textbf{53}:1--9, 2017.

\bibitem{banerjee2018mathematical}
S Banerjee;
%\newblock Mathematical model of relativistic anisotropic compact stellar model
%	admitting linear equation of state.
\newblock {\em Communications in Theoretical Physics}, \textbf{70}:585--592, 2018.


\bibitem{prasad2022anisotropic}
A K Prasad  and J Kumar;
%\newblock Anisotropic relativistic fluid spheres with a linear equation of
%	state.
\newblock {\em New Astronomy}, \textbf{95}:1--18, 2022.

\bibitem{patel2023new}
R Patel, B S Ratanpal, and D M Pandya;
%\newblock New charged anisotropic solution on paraboloidal spacetime.
\newblock {\em Astrophysics and Space Science}, \textbf{368}:1--11, 2023.

\bibitem{sharma2013relativistic}
R Sharma and B S Ratanpal;
%\newblock Relativistic stellar model admitting a quadratic equation of state.
\newblock {\em International Journal of Modern Physics D}, \textbf{22}:1--17,
2013.

\bibitem{bhar2016anisotropic}
P Bhar, K N Singh, and T Manna;
%\newblock Anisotropic compact star with tolman iv gravitational potential.
\newblock {\em Astrophysics and Space Science}, \textbf{361}:284--294, 2016.

\bibitem{bhar2016new}
P Bhar and B S Ratanpal;
%\newblock A new anisotropic compact star model having matese \& whitman mass
%function.
\newblock {\em Astrophysics and Space Science}, \textbf{361}:217--224, 2016.

\bibitem{bhar2015dark}
P Bhar and F Rahaman;
%\newblock The dark energy star and stability analysis.
\newblock {\em The European Physical Journal C}, \textbf{75}:1--12, 2015.

\bibitem{murad2015some}
M H Murad and S Fatema;
%\newblock Some new wyman--leibovitz--adler type static relativistic charged
%	anisotropic fluid spheres compatible to self-bound stellar modeling.
\newblock {\em The European Physical Journal C}, \textbf{192}:1--21, 2015.

\bibitem{thirukkanesh2018anisotropic}
S Thirukkanesh, F C Ragel, R Sharma, and S Das;
%\newblock Anisotropic generalization of well-known solutions describing
%relativistic self-gravitating fluid systems: an algorithm.
\newblock {\em The European Physical Journal C}, \textbf{78}:1--9, 2018.

\bibitem{sharma2007class}
R Sharma and S D Maharaj;
%\newblock A class of relativistic stars with a linear equation of state.
\newblock {\em Monthly Notices of the Royal Astronomical Society},
\textbf{375}:1265--1268, 2007.

\bibitem{thomas2017anisotropic}
V O Thomas and D M Pandya;
%\newblock Anisotropic compacts stars on paraboloidal spacetime with linear
%equation of state.
\newblock {\em The European Physical Journal A}, \textbf{53}:1--9, 2017.

\bibitem{bhar2016anisotropic}
P Bhar, K N Singh, and T Manna;
%\newblock Anisotropic compact star with tolman iv gravitational potential.
\newblock {\em Astrophysics and Space Science}, \textbf{361}:284--294, 2016.

\bibitem{sunzu2014charged}
J M Sunzu, S D Maharaj, and S Ray ;
%\newblock Charged anisotropic models for quark stars.
\newblock {\em Astrophysics and Space Science}, \textbf{352}:719--727, 2014.

\bibitem{komathiraj2007analytical}
K Komathiraj and S D Maharaj;
%\newblock Analytical models for quark stars.
\newblock {\em International Journal of Modern Physics D}, \textbf{16}:1803--1811,
2007.

\bibitem{bhar2015singularity}
P Bhar;
%\newblock Singularity-free anisotropic strange quintessence star.
\newblock {\em Astrophysics and Space Science}, \textbf{356}:309--318, 2015.

\bibitem{bhar2017compact}
P Bhar, K N Singh, and D N Pant;
%\newblock Compact star modeling with quadratic equation of state in tolman vii
%space--time.
\newblock {\em Indian Journal of Physics}, \textbf{91}:701--709, 2017.

\bibitem{bhar2016modelling}
P Bhar, S K Maurya, Y K Gupta, and T Manna;
%\newblock Modelling of anisotropic compact stars of embedding class one.
\newblock {\em The European Physical Journal A}, \textbf{52}:312--322, 2016.

\bibitem{das2019new}
S Das, F Rahaman, and L Baskey;
%\newblock A new class of compact stellar model compatible with observational
%data.
\newblock {\em The European Physical Journal C}, \textbf{79}:853--865, 2019.

\bibitem{das2021modeling}
S Das, K N Singh, L Baskey, F Rahaman, and A K Aria;
%\newblock Modeling of compact stars: an anisotropic approach.
\newblock {\em General Relativity and Gravitation}, \textbf{53}:1--32, 2021.

\bibitem{ratanpal2023anisotropic}
B S Ratanpal and R Patel;
%\newblock Anisotropic approach: compact star as generalized model.
\newblock {\em Astrophysics and Space Science}, \textbf{368}:1--10, 2023.

\bibitem{tikekar2007relativistic}
R Tikekar and  K Jotania;
%\newblock On relativistic models of strange stars.
\newblock {\em Pramana}, \textbf{68}:397--406, 2007.

\bibitem{herrera1992cracking}
L Herrera;
%\newblock Cracking of self-gravitating compact objects.
\newblock {\em Physics Letters A}, \textbf{165}:206--210, 1992.

\bibitem{finch1998review}
M R Finch and  J E F Skea;
%\newblock A review of the relativistic static fluid sphere.
\newblock {\em preprint available on the World Wide Web at http://edradour.
	symbcomp. uerj. br/pubs. html}, 1998.

\bibitem{delgaty1998physical}
M S R Delgaty and K Lake;
%\newblock Physical acceptability of isolated, static, spherically symmetric,
%perfect fluid solutions of einstein's equations.
\newblock {\em Computer Physics Communications}, \textbf{115}:395--415, 1998.

\bibitem{abreu2007sound}
H Abreu, H Hern{\'a}ndez, and L A N{\'u}nez;
%\newblock Sound speeds, cracking and the stability of self-gravitating
%anisotropic compact objects.
\newblock {\em Classical and Quantum Gravity}, \textbf{24}:4631--4645, 2007.

\bibitem{ratanpal2020cracking}
B S Ratanpal;
%\newblock Cracking and stability of non-rotating relativistic spheres with
%anisotropic internal stresses.
\newblock {\em IOP SciNotes}, \textbf{1}:1-8, 2020.

\bibitem{bondi1964contraction}
H Bondi;
%\newblock The contraction of gravitating spheres.
\newblock {\em Proceedings of the Royal Society of London. Series A.
	Mathematical and Physical Sciences}, \textbf{281}:39--48, 1964.



